Monge, Bregman and Occam: Interpretable Optimal Transport in High-Dimensions with Feature-Sparse Maps

Optimal transport (OT) theory focuses, among all maps $T:\mathbb{R}^d\rightarrow \mathbb{R}^d$ that can morph a probability measure onto another, on those that are the ``thriftiest'', i.e. such that the averaged cost $c(x, T(x))$ between $x$ and its image $T(x)$ be as small as possible. Many computational approaches have been proposed to estimate such Monge maps when $c$ is the $\ell_2^2$ distance, e.g., using entropic maps [Pooladian'22], or neural networks [Makkuva'20, Korotin'20]. We propose a new model for transport maps, built on a family of translation invariant costs $c(x, y):=h(x-y)$, where $h:=\tfrac{1}{2}\|\cdot\|_2^2+\tau$ and $\tau$ is a regularizer. We propose a generalization of the entropic map suitable for $h$, and highlight a surprising link tying it with the Bregman centroids of the divergence $D_h$ generated by $h$, and the proximal operator of $\tau$. We show that choosing a sparsity-inducing norm for $\tau$ results in maps that apply Occam's razor to transport, in the sense that the displacement vectors $\Delta(x):= T(x)-x$ they induce are sparse, with a sparsity pattern that varies depending on $x$. We showcase the ability of our method to estimate meaningful OT maps for high-dimensional single-cell transcription data, in the $34000$-$d$ space of gene counts for cells, without using dimensionality reduction, thus retaining the ability to interpret all displacements at the gene level.

==> sections/bin.tex <==
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=.4\textwidth]{figures/illustration.pdf}
%     \caption{Illustration of the entropic map estimator with the elastic $\ell_1$ norm in 2d.
%     %
%     Here, the orange points are the $\bx_i$, the blue points are the $\by_j$.
%     %
%     The points in black are transported to the red point with the map $T_{h, \varepsilon}$ computed on this problem. We see that some transports only occur along one dimension, illustrating the sparsity of the displacement. The green rectangle is the zone such that $T_{h, \varepsilon}(\bx) = \bx$.}
%     \label{fig:illust}
% \end{figure}

% We propose now approaches to define a cost $h$ that directly impact the type of displacements obtained in Definition~\ref{def:emap}. We propose two methods to do so, which can be seen as a generalization of the canonical choice $h=\tfrac{1}{2}\|\cdot\|_2^2$ used by \citep{Bre91} and widely adopted in optimal transport. The first approach consists simply in choosing a different norm inside the square, different from $\|\cdot\|_2$. The second consists in adding to the squared $\ell_2$ term an additional sparsifying term, in the spirit of the elastic-net regularization~\citep{zou2005regularization}.

% \subsection{Squared-Norms and their Conjugate}
% Several norms relevant to sparsity admit a closed form dual norm. We exploit the result that the Legendre transform of a squared-norm is tightly connected to its dual norm to define $h$. One has indeed that
% $$(\tfrac{1}{2}\|\cdot\|^2)^* = \tfrac{1}{2}\|\cdot\|_*^2$$ \citep[Example 3.27]{boyd2004convex}. As a result, we can show that setting $h$ to be exactly $\frac{1}{2}\|\cdot\|^2$, the the subdifferential of $h^*$ is given by the rescaled sub-differential of $\|\cdot\|_*$:
% $$
% \partial h^*(z) = \|z\|_* \partial \|z\|_*
% $$


